LongGenBench: Long-context Generation Benchmark

Current long-context benchmarks primarily focus on retrieval-based tests, requiring Large Language Models (LLMs) to locate specific information within extensive input contexts, such as the needle-in-a-haystack (NIAH) benchmark. Long-context generation refers to the ability of a language model to generate coherent and contextually accurate text that spans across lengthy passages or documents. While recent studies show strong performance on NIAH and other retrieval-based long-context benchmarks, there is a significant lack of benchmarks for evaluating long-context generation capabilities. To bridge this gap and offer a comprehensive assessment, we introduce a synthetic benchmark, LongGenBench, which allows for flexible configurations of customized generation context lengths. LongGenBench advances beyond traditional benchmarks by redesigning the format of questions and necessitating that LLMs respond with a single, cohesive long-context answer. Upon extensive evaluation using LongGenBench, we observe that: (1) both API accessed and open source models exhibit performance degradation in long-context generation scenarios, ranging from 1.2% to 47.1%; (2) different series of LLMs exhibit varying trends of performance degradation, with the Gemini-1.5-Flash model showing the least degradation among API accessed models, and the Qwen2 series exhibiting the least degradation in LongGenBench among open source models.

==> temp_fig.tex <==
% \section{Importance of Long-Context Generation and \method{} Evaluation}
% \label{sec:importance}

% \paragraph{Definition of Long-Context Generation:}
% Long-context generation refers to the ability of a language model to generate coherent and contextually accurate text that spans across a lengthy passage or document. This capability involves maintaining the thematic continuity, logical flow, and consistency of details over extended sequences of text, which can include multiple paragraphs, pages, or even entire documents.

% \paragraph{Importance of Long-Context Generation:}
% The significance of long-context generation lies in its wide array of applications where the ability to understand and generate extensive and coherent text is crucial. Here are some key scenarios highlighting its importance:

% \begin{itemize}
%     \item \textbf{Scientific Research and Documentation:} Generating detailed scientific reports, papers, and documentation requires models to synthesize information from various sections cohesively. Long-context generation ensures that references, hypotheses, and conclusions are logically connected across multiple pages.
    
%     \item \textbf{Legal Document Analysis:} Legal documents are lengthy and complex, requiring careful consideration of context across numerous clauses and sections. A model proficient in long-context generation can assist in drafting legal documents, summarizing cases, and extracting relevant information without losing the established context.
    
%     \item \textbf{Customer Service and Support:} Effective customer service involves understanding the full history of customer interactions. Long-context generation allows models to manage multi-turn dialogues, remembering previous interactions to resolve issues more efficiently.
    
%     \item \textbf{Content Creation and Storytelling:} For content creators and storytellers, generating cohesive narratives over multiple chapters or segments is essential. Long-context generation helps maintain character development, plot consistency, and thematic elements throughout the entire piece.
    
%     \item \textbf{Educational Tools and Tutoring:} Personalized tutoring systems benefit from long-context generation by keeping track of a student's progress and past interactions, allowing for tailored and effective teaching strategies.
    
%     \item \textbf{Healthcare and Medical Records:} Managing patient records and generating comprehensive medical reports require maintaining context over long documents. Long-context generation ensures that all relevant medical history, diagnoses, and treatments are considered, providing accurate and holistic patient care.
% \end{itemize}

% \paragraph{Lack of Existing Benchmarks:}
% Despite its importance, there is currently a lack of benchmarks specifically designed to evaluate long-context generation capabilities of language models. Existing benchmarks typically focus on short-context tasks, assessing the model's performance on generating responses to individual questions or short prompts. These benchmarks do not adequately measure the model's ability to maintain coherence and accuracy over extended sequences of text.

% \paragraph{Introduction of \method{}:}
% To address this gap, we introduce \method{}, a benchmark framework specifically designed to evaluate long-context generation capabilities of language models. \method{} involves generating responses to a set of $K$ questions concatenated into a single long input prompt, assessing the model's ability to generate coherent and contextually accurate answers over an extended passage. This evaluation framework provides a comprehensive assessment of a model's performance in real-world scenarios where long-context generation is crucial.

% \method{}'s evaluation involves measuring how well models can handle various long-context tasks, such as those in scientific research, legal document analysis, customer service, content creation, education, and healthcare. By rigorously testing models on these tasks, \method{} highlights the strengths and weaknesses of different models in managing long-context generation, guiding the development and selection of models better suited for applications requiring this capability.



% \definecolor{prompt}{HTML}{6085e4}
% \definecolor{label_color}{HTML}{f19eac}

% \begin{table*}[h]
%     \centering
%     \begin{tabular}{p{0.15\linewidth}|p{0.75\linewidth}}
%     \toprule
%     \textbf{Method} & \textbf{Template} \\ 
%     \midrule
    
%     Baseline & \textcolor{violet}{\{System Prompt\}} \\
%         &\textcolor{prompt}{\{CoT Question\_1\}}\textcolor{orange}{\{CoT Asnwer\_1\}} \\ 
%         &$\cdots$ \\
%         &\textcolor{prompt}{\{CoT Question\_8\}}\textcolor{orange}{\{CoT Asnwer\_8\}} \\ 
%         & \textcolor{label_color}{\{Real Question\}} \\ \midrule
    
%     \method{}&  \textcolor{violet}{\{System Prompt\}}  \\
%         &\textcolor{prompt}{\{CoT Question\_1\}}$\cdots$\textcolor{prompt}{\{CoT Question\_8\}} \\
%         &\textcolor{orange}{\{CoT Asnwer\_1\}}$\cdots$\textcolor{orange}{\{CoT Asnwer\_8\}} \\
%         &\textcolor{label_color}{\{Real Question\_1\}}  $\cdots$  \textcolor{label_color}{\{Real Question\_$K$\}} \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{Model chat templates. The table compares the baseline method with the \method{} approach in terms of chat templates used for model interactions. In the baseline method, the system prompt is followed by a series of chain-of-thought (CoT) questions and answers, ending with a real question. In contrast, the \method{} approach involves concatenating multiple CoT questions and answers, followed by multiple real questions, to prompt the model for long-context responses. This approach helps to evaluate the model's ability to generate coherent and accurate long-context answers across a series of related questions.}
%     \label{tab:model_template}
% \end{table*}



% % \begin{wrapfigure}{r}{0.44\textwidth}
% \definecolor{chatcolor1}{HTML}{FFFACD} % 8FFED2
% \definecolor{shadecolor}{gray}{0.95}
% \definecolor{label_color}{HTML}{f19eac}
% \definecolor{prompt}{HTML}{6085e4}
% \definecolor{shadecolor_1}{gray}{0.55}
% \begin{figure}[htbp]
% \centering
% \tikzstyle{every node}=[font=\small,scale=0.9]
% \begin{tikzpicture}
%     \footnotesize
%     \definecolor{chatcolor1}{HTML}{FFFACD} % 8FFED2
%     \definecolor{shadecolor}{gray}{0.95}
%     \definecolor{label_color}{HTML}{f19eac}
%     \definecolor{prompt}{HTML}{6085e4}
%     \definecolor{shadecolor_1}{gray}{0.55}
%     \fontfamily{cmss}\selectfont
%     % fill opacity=0.7, text opacity=1 透明度
%     % line width=0.5mm, 边框粗细

%     \node[align=left, text width=0.6\textwidth, fill=shadecolor, rounded corners=1mm, draw=black, line width=0.5mm, fill opacity=0.7, text opacity=1, anchor=north west] (node1) at (0,0) {
%         \textcolor{prompt}{$\#$ $K$ questions in order} \\ 
%         \textbf{Input:} \\
%         Question 1: A basket contains 25 oranges among which 1 is bad, 20\% are unripe, 2 are sour and the rest are good. How many oranges are good? \\ 
%         \vspace{1\baselineskip}       
%         Question 2: A raspberry bush has 6 clusters of 20 fruit each and 67 individual fruit scattered across the bush. How many raspberries are there total? \\
%         \vspace{1\baselineskip}        
%         Question 3: Lloyd has an egg farm. His chickens produce 252 eggs per day and he sells them for \$2 per dozen. How much does Lloyd make on eggs per week? \\ 
%         \textcolor{shadecolor_1}{$\cdots$}	\\
%         \textcolor{shadecolor_1}{$\cdots$}	\\
%         Question $K$:John buys twice as many red ties as blue ties.  The red ties cost 50\% more than blue ties.  He spent \$200 on blue ties that cost \$40 each. How much did he spend on ties? \\
%     };
%     \node[align=left, text width=0.5\textwidth, fill=chatcolor1, rounded corners=1mm, draw=black, line width=0.5mm, fill opacity=0.7, text opacity=1, anchor=north east] (node2) at ($(node1.south -| {0.6\textwidth,0}) + (0,-0.2cm)$) {
%    \textcolor{prompt}{$\#$ $K$ answers in order} \\ 
%     \textbf{Output:} \\
%         Answer 1: There are 25 oranges in total. 1 is bad. 20\% of 25 is 25 x 0.20 = 5 unripe. $\cdots$ The answer is 17. \emojicheck \\
%         \vspace{1\baselineskip}       
%         Answer 2: There are 6 clusters of 20 fruit each. So 6 x 20 = 120 raspberries $\cdots$ The answer is 187. \emojicheck \\
%         \vspace{1\baselineskip}       
%         Answer 3: Lloyd's chickens produce 252 eggs per day. A dozen is 12 eggs, $\cdots$ The answer is \$294. \emojicheck \\
%         \textcolor{shadecolor_1}{$\cdots$}	\\
%         \textcolor{shadecolor_1}{$\cdots$}	\\
%         Answer $K$: He spent \$200 on blue ties that cost \$40 each.$\cdots$ The answer is \$800. \emojicheck 
%     };

%     \draw[rounded corners=3mm, draw=none, fill=none] ($(node1.north west)+(-0.2,0.2)$) rectangle ($(node2.south east)+(0.2,-0.2)$);    
% \end{tikzpicture}
% % \vspace{-10pt}
% \caption{Neeld-in-a-haystack figure.}  
% \label{fig:app_basline}
% \end{figure}
% % \end{wrapfigure}


% \begin{figure}[htbp]
% \centering
% \tikzstyle{every node}=[font=\small,scale=0.9]
% \begin{tikzpicture}
%     \footnotesize
%     \definecolor{chatcolor1}{HTML}{FFFACD} % 8FFED2
%     \definecolor{shadecolor}{gray}{0.95}
%     \definecolor{label_color}{HTML}{f19eac}
%     \definecolor{shadecolor_1}{gray}{0.55}
%     \fontfamily{cmss}\selectfont
%     % fill opacity=0.7, text opacity=1 透明度
%     % line width=0.5mm, 边框粗细

%     \node[align=left, text width=0.6\textwidth, fill=shadecolor, rounded corners=1mm, draw=black, line width=0.5mm, fill opacity=0.7, text opacity=1, anchor=north west] (node1) at (0,0) {
%         \textcolor{prompt}{$\#$ Retrieval task} \\ 
%         \textbf{Input:} \\
%         \textcolor{shadecolor_1}{(essay...)}\\
%         One of the special magic number for long-context is: \textcolor{label_color}{12345}.\\
%         \textcolor{shadecolor_1}{(essay...)}\\
%         \textbf{Question:} \\ 
%         What is the special magic number for long-context mentioned in the provided text? \\
%     };
%     \node[align=left, text width=0.5\textwidth, fill=chatcolor1, rounded corners=1mm, draw=black, line width=0.5mm, fill opacity=0.7, text opacity=1, anchor=north east] (node2) at ($(node1.south -| {0.6\textwidth,0}) + (0,-0.2cm)$) {
%     \textbf{Output:} \\
%       \textcolor{label_color}{12345}  \emojicheck
%     };

%     \draw[rounded corners=3mm, draw=none, fill=none] ($(node1.north west)+(-0.2,0.2)$) rectangle ($(node2.south east)+(0.2,-0.2)$);    
% \end{tikzpicture}
% % \vspace{-10pt}
% \caption{LongerBench figure.}  
% \label{fig:app_basline}
% \end{figure}
% % \end{wrapfigure}



% \begin{figure}[htbp]
% \centering
% \tikzstyle{every node}=[font=\small,scale=0.9]
% \begin{tikzpicture}
%     \footnotesize
%     \definecolor{chatcolor1}{HTML}{FFFACD} % 8FFED2
%     \definecolor{shadecolor}{gray}{0.95}
%     \definecolor{label_color}{HTML}{f19eac}
%     \definecolor{label_color_2}{HTML}{7ccf4d}
%     \definecolor{shadecolor_1}{gray}{0.55}
%     \fontfamily{cmss}\selectfont
%     % fill opacity=0.7, text opacity=1 透明度
%     % line width=0.5mm, 边框粗细

%     \node[align=left, text width=0.6\textwidth, fill=shadecolor, rounded corners=1mm, draw=black, line width=0.5mm, fill opacity=0.7, text opacity=1, anchor=north west] (node1) at (0,0) {
%         \textcolor{prompt}{$\#$ Understanding task} \\ 
%         \textbf{Input:} \\
%         \textcolor{shadecolor_1}{(essay start...)}\\
%         Bhagirathi (film) is a 2012 Indian Kannada drama film written and directed by \textcolor{label_color_2}{Baraguru Ramachandrappa}. \\
%         \textcolor{shadecolor_1}{(essay...)}\\
%         \textcolor{label_color_2}{Biography Ramachandrappa} was born to Kenchamma and Rangadasappa in Baraguru village in the \textcolor{label_color}{Tumkur} district. \\
%         \textcolor{shadecolor_1}{($\cdots$ essay end)}\\
%         \textbf{Question:} \\ 
%         What is the \textcolor{label_color}{place of birth} of the \textcolor{label_color_2} {director} of film Bhagirathi (Film)? \\

%     };
%     \node[align=left, text width=0.5\textwidth, fill=chatcolor1, rounded corners=1mm, draw=black, line width=0.5mm, fill opacity=0.7, text opacity=1, anchor=north east] (node2) at ($(node1.south -| {0.6\textwidth,0}) + (0,-0.2cm)$) {
%     \textbf{Output:} \\
%       \textcolor{label_color}{Tumkur}  \emojicheck
%     };

%     \draw[rounded corners=3mm, draw=none, fill=none] ($(node1.north west)+(-0.2,0.2)$) rectangle ($(node2.south east)+(0.2,-0.2)$);    
% \end{tikzpicture}
% % \vspace{-10pt}
% \caption{Neeld-in-a-haystack figure.}  
% \label{fig:app_basline}
% \end{figure}

% % \begin{figure}[htp]
% % \centering
% % \tikzstyle{every node}=[font=\small,scale=0.9]
% % \begin{tikzpicture}
% %     \footnotesize
% %     \definecolor{chatcolor1}{HTML}{FFFACD} % 8FFED2
% %     \definecolor{shadecolor}{gray}{0.95}
% %     \definecolor{shadecolor_1}{gray}{0.55}
% %     \fontfamily{cmss}\selectfont
% %     % fill opacity=0.7, text opacity=1 透明度
% %     % line width=0.5mm, 边框粗细

% %     \node[align=left, text width=0.888\textwidth, fill=shadecolor, rounded corners=1mm, draw=black, line width=0.5mm, fill opacity=0.7, text opacity=1, anchor=north west] (node1) at (0,0) {
% %         \textbf{Input:} \\
% %         \textcolor{shadecolor_1}{(essay...)}\\
% %         One of the special magic number for long-context is: 12345.\\
% %         \textcolor{shadecolor_1}{(essay...)}\\
% %         \textbf{Question:} \\ 
% %         What is the special magic number for long-context mentioned in the provided text? \\
% %     };
% %     \node[align=left, text width=0.9\textwidth, fill=chatcolor1, rounded corners=1mm, draw=black, line width=0.5mm, fill opacity=0.7, text opacity=1, anchor=north east] (node2) at ($(node1.south -| {0.88\textwidth,0}) + (0,-0.2cm)$) {
% %     \textbf{Answer:} \\
% %      12345  \emojicheck
% %     };

% %     \draw[rounded corners=3mm, draw=none, fill=none] ($(node1.north west)+(-0.2,0.2)$) rectangle ($(node2.south east)+(0.2,-0.2)$);    
% % \end{tikzpicture}
% % % \vspace{-10pt}
% % \caption{Neeld-in-a-haystack figure.}  
% % \label{fig:app_basline}
% % \end{figure}

